Rainbow cycles in flip graphs

The flip graph of triangulations has as vertices all triangulations of a convex $n$-gon, and an edge between any two triangulations that differ in exactly one edge. An $r$-rainbow cycle in this graph is a cycle in which every inner edge of the triangulation appears exactly $r$ times. This notion of a rainbow cycle extends in a natural way to other flip graphs. In this paper we investigate the existence of $r$-rainbow cycles for three different flip graphs on classes of geometric objects: the aforementioned flip graph of triangulations of a convex $n$-gon, the flip graph of plane trees on an arbitrary set of $n$ points, and the flip graph of non-crossing perfect matchings on a set of $n$ points in convex position. In addition, we consider two flip graphs on classes of non-geometric objects: the flip graph of permutations of $\{1,2,\dots,n\}$ and the flip graph of $k$-element subsets of $\{1,2,\dots,n\}$. In each of the five settings, we prove the existence and non-existence of rainbow cycles for different values of $r$, $n$ and~$k$.

==> graphics/match8.tex <==
% draw the given number of points equidistantly on a circle
% and call them (1),...,(n)
\newcommand{\matching}[1]{
\foreach \i in {1,...,#1} {
  \node[node_black] (\i) at (-\i*360/#1-90+180/#1:1.5) {};
  \draw (-\i*360/#1-90+180/#1:1.8) node {$\i$};
}
}

\begin{tikzpicture}[scale=1]

\matching{8}
    
\path[line_solid] (1) to (8);
\path[line_solid] (2) to (7);
\path[line_solid] (3) to (4);
\path[line_solid] (5) to (6);

\path[line_dashed] (2) to (5);
\path[line_dashed] (6) to (7);

\end{tikzpicture}

==> graphics/match8r2_9n.tex <==
\begin{tikzpicture}[scale=0.42]

\matching{16}

\path[line_solid] (1) to (16);
\path[line_solid] (2) to (3);
\path[line_solid] (4) to (15);
\path[line_solid] (5) to (6);
\path[line_solid] (7) to (8);
\path[line_solid] (9) to (10);
\path[line_solid] (11) to (14);
\path[line_solid] (12) to (13);

\draw (0,0) node {$M'$};

\end{tikzpicture}

